Abusing Phone Numbers and Cross-Application Features for Crafting Targeted Attacks

With the convergence of Internet and telephony, new applications (e.g., WhatsApp) have emerged as an important means of communication for billions of users. These applications are becoming an attractive medium for attackers to deliver spam and carry out more targeted attacks. Since such applications rely on phone numbers, we explore the feasibility, automation, and scalability of phishing attacks that can be carried out by abusing a phone number. We demonstrate a novel system that takes a potential victim's phone number as an input, leverages information from applications like Truecaller and Facebook about the victim and his / her social network, checks the presence of phone number's owner (victim) on the attack channels (over-the-top or OTT messaging applications, voice, e-mail, or SMS), and finally targets the victim on the chosen channel. As a proof of concept, we enumerate through a random pool of 1.16 million phone numbers. By using information provided by popular applications, we show that social and spear phishing attacks can be launched against 51,409 and 180,000 users respectively. Furthermore, voice phishing or vishing attacks can be launched against 722,696 users. We also found 91,487 highly attractive targets who can be attacked by crafting whaling attacks. We show the effectiveness of one of these attacks, phishing, by conducting an online roleplay user study. We found that social (69.2%) and spear (54.3%) phishing attacks are more successful than non-targeted phishing attacks (35.5%) on OTT messaging applications. Although similar results were found for other mediums like e-mail, we demonstrate that due to the significantly increased user engagement via new communication applications and the ease with which phone numbers allow collection of information necessary for these attacks, there is a clear need for better protection of OTT messaging applications.

==> vishing.tex <==
%!TEX root = main.tex
%\section{Other Attack Channels}
%In this section, we focus on other attacks that can be crafted with the collected data. We highlight the possibility of crafting vishing attacks (see Section~\ref{sec:vishing}) on traditional telephony channel using phone number as a unique identifier 
%and exploiting the integrity of information provided by \caller. 
%We also provide an early evidence of crafting targeted whaling attacks (see Section~\ref{sec:whaling}), launched on specific set of phone numbers, called vanity numbers. 
%%In addition, we focus on other attacks that can be carried out by abusing phone numbers.
%
%\subsection{Launching Vishing Attacks by Undermining the Integrity of Information provided by Caller ID Applications} \label{sec:vishing}
%With the advent of cheap Voice over IP calls, 
%phishing attacks have evolved from web-based 
%attacks to targeted telephone-based attacks, called 
%as voice phishing (vishing)~\cite{voice_phishing}
%conducted by exploiting the trust in voice communication. 
%In vishing, scammers either call or lure people to call 
%phone numbers controlled by them, and try to collect personal information 
%about the owner of a phone number for the purpose of committing 
%fraud~\cite{vishing_attack_4,vishing_attack_3}.
%One of the reason why vishing attacks are successful is due to the lack of  
%intelligence about the calling phone number itself. 
%To avoid falling a victim to these targeted attacks and to know more about the 
%incoming phone number, cloud-based caller identification services 
%are emerging to help in getting additional information about the caller. 
%Millions of people are using such applications, 
%namely Truecaller~\cite{truecaller}, Facebook's Hello~\cite{hello}, and Whitepages Caller ID and Block~\cite{current_caller_id}. 
%In general, these applications allow an individual to register 
%using his~/~her phone number and help in identifying 
%the caller by showing the information (like name) from their respective databases.
%\Caller also gather information from social networking sites to collect 
%more information about the caller. 
%
%We explored the feasibility of targeted vishing attacks by collecting 
%information from one of the \caller, Truecaller, and 
%leveraging more personal information about the victim from Facebook. 
%This is possible due to less reliable 
%information
%provided by these crowd-sourced \caller, unlike CNAM services that are verified to some extent by service providers~\cite{moss2006method}. 
%Scammers can undermine such an application 
%to vish their victims. 
%The information can be exploited to conduct targeted social engineering / vishing attacks.
%Specifically, a) scammers can register a phone number (controlled
%by him / her) as a trusted bank / company / organization in which a user is interested in or is dealing with; 
%b) spoof one of the already registered phone numbers with
%the \caller and call victims such that the call
%appears to come from a real entity.
%\paragraph{Fake Registration}
%An attacker can add spurious information in \caller fairly easily, 
%thus compromising the integrity of the information provided by them to launch vishing attacks. 
%Associating an identity with a phone number increases the trust of an individual and likelihood to pick a call. 
%Since \caller do not have a mechanism 
%for verification of the users' details, and rely on the information provided 
%by the user while registering, it is easy for an attacker to abuse this trust. 
%For example, an attacker can register as multiple fake banks on \caller.
%For registration, he needs a smartphone device with working phone connection. 
%It is a manual process where a short SMS code is sent from \caller to verify the phone number.
%Since the number of banks are limited, it is not difficult for the attacker to do this manually.
%Attacker does not know the bank of all these victims, therefore, 
%the attacker can target a large user population to achieve a good success rate. 
%He can generate millions of automated VoIP calls at low cost, 
%as shown in the past~\cite{griffin2008vishing}.
%
%To make the attack look more authentic, 
%fake social media profiles can be created 
%and linked to \caller while registering an account on it. 
%Further, fetching details about the victim (person to be called) 
%from social networking 
%sites can increase the success of such attacks. 
%Since vishing attacks are already known to be 
%successful~\cite{vishing_attack_4, vishing_attack_2}, we believe success rate of 
%targeted attacks would be higher or at-least equivalent. 
%Figure~\ref{fig:tc_hdfc} shows fake registration as HDFC bank by exploiting one of the \caller, %Truecaller.
%We only use HDFC Bank as an example, but any name / entity can be used.

%\begin{figure}[ht]
%\begin{center}
%\includegraphics[width=3.35cm, trim=4.9cm 6.8cm 3.6cm 0cm, clip]{figs/tc_register.png}
%\caption{Example showing fake registration on Truecaller as HDFC Bank.}
%\label{fig:tc_hdfc}
%\end{center}
%\end{figure}

%We demonstrated how integrity of the information provided by various \caller can be compromised. Figure~\ref{fig:tc}
%shows incoming call showing fake ``HDFC Bank" on various \caller; Truecaller, 
%Whitepages Caller ID and Block, Facebook's Hello application, Whoscall Caller
%ID and Block, and Contactive.
%
%\begin{figure*}[ht]
%%\subcapraggedrighttrue
%\begin{center}
%\subfigure[Truecaller]
%{ \label{fig:truecaller}
%%\includegraphics[width=7cm,height=7cm,keepaspectratio]{figs/register.png}
%\includegraphics[width=3.35cm, trim=4.9cm 6.8cm 3.6cm 0cm, clip]{figs/tc_call.png}
%}
%\subfigure[Whitepages Caller ID \& Block]
%{ \label{fig:whitepages}
%%\includegraphics[width=7cm,height=7cm,keepaspectratio]{figs/register.png}
%\includegraphics[width=3.35cm, trim=4.9cm 6.8cm 3.6cm 0cm, clip]{figs/tc_call_whitepages.png}
%}
%\subfigure[Facebook's Hello]
%{ \label{fig:hello}
%%\includegraphics[width=7cm,height=7cm,keepaspectratio]{figs/register.png}
%\includegraphics[width=3.35cm, trim=4.9cm 6.8cm 3.6cm 0cm, clip]{figs/tc_call_hello.png}
%}
%\subfigure[Whoscall-Caller ID and Block]
%{ \label{fig:whoscall}
%%\includegraphics[width=7cm,height=7cm,keepaspectratio]{figs/register.png}
%\includegraphics[width=3.35cm, trim=4.9cm 6.8cm 3.6cm 0cm, clip]{figs/tc_call_line.png}
%}
%%\subfigure[Contactive]
%%{ \label{fig:contactive}
%%\includegraphics[width=7cm,height=7cm,keepaspectratio]{figs/register.png}
%%\includegraphics[width=3.35cm, trim=4.9cm 6.8cm 3.6cm 0cm, clip]{figs/tc_call_contactive.png}
%%}
%\caption{Incoming call from fake HDFC Bank (example in our case) on various \caller.}
%\label{fig:tc}
%\end{center}
%\end{figure*}


%\paragraph{Caller ID spoofing}
%Another form of attack uses caller ID spoofing which can be carried out by imitating already registered 
%phone numbers or other phone numbers
%whose details were uploaded by \caller exploiting address book syncing feature. 
%As a user must have entered some details about 
%him / her while registering, it makes him / her a more likely target, 
%than an unknown phone number flashing on the screen. 
%
%Personal information for 722,696 users was found on Truecaller against 1,162,696 
%phone numbers searched. Vishing attacks can be crafted against the owners of these phone numbers.
%We could 
%extract Facebook ID's for 122,696 users. 
%Using Facebook Graph API, we obtained following 
%details for these users: gender (112,880), relationship 
%status (57,755), work details (92,352), school 
%information (110,426), employer details (106,746), 
%birthday (9,728), and hometown (80,979). 
%The collated information can be used to increase 
%the success rate of targeted vishing attacks.

%\subsection{Launching Whaling Attacks on \ott and Traditional Telephony Channels} \label{sec:whaling}
%Whaling attacks~\cite{whaling} that are directed specifically at senior executives or other high-profile 
%individuals within a business, government, or other organization, can be crafted on \ott. It uses 
%the same technique as above mentioned targeted phishing / vishing attacks but the intended victims are people with high influence
%or high-net-worth individuals.
%In India, there is a particular set of phone numbers reserved by mobile operators for politicians, 
%bureaucrats, and people willing to invest large amount of money to get a phone number. 
%They are called Vanity / VIP / Fancy numbers and follow a specific pattern~\cite{vanity-pattern}. 
%It could 
%be one digit repeated several times, 99999-xxxxx or xx-8888-xxxx; 
%two digits, xx-85-85-85-xx; or in different orders, xx-123-123-xx or xx-11-112233. 
%The main advantage of vanity phone numbers over standard phone numbers is 
%increased memorability. Since they 
%are bought at higher price, owners of these phone numbers can be assumed as people with high influence~\cite{vanity}. 
%For very special numbers, network providers 
%host auctions online where people can purchase these numbers~\cite{bsnl-auction}. 
%Using only vanity numbers in the address book, attackers can launch 
%whaling attacks that only targets 
%HNIs (High-net-worth individuals) by sending them 
%targeted or non-targeted phishing messages or initiating vishing calls.

%We looped through the ``patterns" available 
%from an e-auction website to enumerate vanity numbers pool~\cite{bsnl-auction}. 
%We initialized our smartphone's address book with 171,323 vanity numbers. 
%They were synced with WhatsApp and 40,223 (23\%) were found 
%on it. We also found 91,487 vanity numbers on Truecaller and 11,286 on Facebook. 
%The information from multiple applications can be aggregated together to craft various targeted attacks as demonstrated above.
%Out of 11,286 vanity numbers that were found on Truecaller and Facebook; we obtained personal information (using Facebook) about owners as follows: gender~(10,246), relationship status~(3,733), birthday~(726), work details~(6,729), school details~(10,994), employer details (9,801), and hometown~(6,952). 
%We manually analyzed Facebook profiles of 100 random vanity number owners to find their occupation details and found director~/~CEO~/~chairman~(10), student~(10), engineer~(12), consultants~(2), business~(5), accountant~/~officer~(8), lecturer~(5), manager~(8), bank officials~(12) for 70 user profiles.
%Detailed analysis of the content (posts and likes) generated by these users can help attackers craft better phishing and vishing attacks against them. 
%Even though people are paying handsomely to protect their privacy, a combination of applications like %Truecaller and Facebook can be used to deanonymize these profiles~\cite{silent_phone_number}. 
%\subsection{Feasibility}
%
%\subsection{Launching Phishing Attacks via E-mails} \label{sec:email_attack}
%Apart from phishing attacks on \ott and other attack channels mentioned above, 
%feasibility of another attack was encountered during the course of this work. 
%E-mail addresses for 81,389 users were obtained from Truecaller against 
%1,162,696 random phone numbers searched. Using Facebook Graph API, we 
%aggregated information like gender, birthday, hometown, work~/~school~/~education details, 
%and relationship status for the user associated to a phone number. Using this information, 
%attacker can choose e-mail as other attack channel to launch personalized and targeted phishing attacks.

